Improving Feasibility via Fast Autoencoder-Based Projections

Enforcing complex (e.g., nonconvex) operational constraints is a critical challenge in real-world learning and control systems. However, existing methods struggle to efficiently enforce general classes of constraints. To address this, we propose a novel data-driven amortized approach that uses a trained autoencoder as an approximate projector to provide fast corrections to infeasible predictions. Specifically, we train an autoencoder using an adversarial objective to learn a structured, convex latent representation of the feasible set. This enables rapid correction of neural network outputs by projecting their associated latent representations onto a simple convex shape before decoding into the original feasible set. We test our approach on a diverse suite of constrained optimization and reinforcement learning problems with challenging nonconvex constraints. Results show that our method effectively enforces constraints at a low computational cost, offering a practical alternative to expensive feasibility correction techniques based on traditional solvers.

==> iclr2026/fab_training_alg_saved.tex <==
\begin{algorithm}[ht]
  \caption{Two-Phase Training Procedure for FAB Feasibility Improvement}
  \label{alg:autoencoder_training}
  \begin{algorithmic}[1]
  \State \textbf{input:} Feasible dataset $\mathcal{T}_{\text{feas}} = \{(y^{(i)}, x^{(i)}) | y^{(i)} \in \mathcal{C}(x^{(i)}) \}$, Discriminator dataset $\mathcal{T}_{\text{disc}} = \{((y^{(i)}, x^{(i)}), c^{(i)}) \}$, Latent space samples $\mathcal{T}_{\text{lat}} = \{z^{(j)} \sim \mathcal{S} \}$
  \Ensure Trained autoencoder parameters $(\gamma, \psi)$

  \State \textbf{Phase 1: Constraint set reconstruction}
  \State Initialize encoder $E_\gamma$, decoder $R_\psi$
  \For{$\text{epoch} = 1$ to $N_1$}
      \For{each batch $(y, x) \in \mathcal{T}_{\text{feas}}$}
          \State $z = E_\gamma(y, x)$
          \State $\hat{y} = R_\psi(z)$
          \State $\mathcal{L}_{\text{recon}} = \| y - \hat{y} \|_2^2$
          \State Update $\gamma, \psi$ by descending $\nabla \mathcal{L}_{\text{recon}}$
      \EndFor
  \EndFor

  \State \textbf{Phase 2: Latent space structuring}
  \State Initialize discriminator $D_\xi$
  \For{$\text{epoch} = 1$ to $N_2$}
      \For{each batch $((y, x), c) \in \mathcal{T}_{\text{disc}}$}
          \State \textbf{Train Discriminator $D_\xi$:}
              \State $\mathcal{L}_{\text{disc}} = - [c \log D_\xi(y, x) + (1 - c) \log(1 - D_\xi(y, x))]$
              \State Update $\xi$ by descending $\nabla \mathcal{L}_{\text{disc}}$

          \State \textbf{Train Autoencoder $(E_\gamma, R_\psi)$:}
          \State $z = E_\gamma(y, x)$
          \State $\hat{y} = R_\psi(z)$
          \State $\mathcal{L}_{\text{recon}} = \| y - \hat{y} \|_2^2$
          \State
          \State Sample a batch $z_{\text{lat}} \in \mathcal{T}_{\text{lat}}$
          \State $\mathcal{L}_{\text{latent}} = -\frac{1}{M} \sum_{j=1}^M \log D_\xi(R_\psi(z_{\text{lat}}^{(j)}))$
          \State $\mathcal{L}_{\text{hinge}} = \frac{1}{N} \sum_{i=1}^{N} [c^{(i)} \max(0, \|z^{(i)}\|_2 - 0.5) + (1 - c^{(i)}) \max(0, 0.5 - \|z^{(i)}\|_2)]$
          \State $J_z = \nabla_z R_\psi(z)$
          \State $\mathcal{L}_{\text{geom}} = \alpha \cdot \text{Var}_{z \sim P_z} [ \log \det(J_z J_z^\top + \varepsilon I_m) ]$
          \State $\mathcal{L}_{\text{struc}} = \lambda_{\text{recon}} \mathcal{L}_{\text{recon}} + \lambda_{\text{latent}} \mathcal{L}_{\text{latent}} + \lambda_{\text{hinge}} \mathcal{L}_{\text{hinge}} + \lambda_{\text{geom}} \mathcal{L}_{\text{geom}}$
          \State Update $\gamma, \psi$ by descending $\nabla \mathcal{L}_{\text{struc}}$
      \EndFor
  \EndFor
  \State \Return Trained parameters $(\gamma, \psi)$
  \end{algorithmic}
  \end{algorithm}
